Global Clipper: Enhancing Safety and Reliability of Transformer-based Object Detection Models

As transformer-based object detection models progress, their impact in critical sectors like autonomous vehicles and aviation is expected to grow. Soft errors causing bit flips during inference have significantly impacted DNN performance, altering predictions. Traditional range restriction solutions for CNNs fall short for transformers. This study introduces the Global Clipper and Global Hybrid Clipper, effective mitigation strategies specifically designed for transformer-based models. It significantly enhances their resilience to soft errors and reduces faulty inferences to ~ 0\%. We also detail extensive testing across over 64 scenarios involving two transformer models (DINO-DETR and Lite-DETR) and two CNN models (YOLOv3 and SSD) using three datasets, totalling approximately 3.3 million inferences, to assess model robustness comprehensively. Moreover, the paper explores unique aspects of attention blocks in transformers and their operational differences from CNNs.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> sec_new/ablation.tex <==
% \section{Ablation}



\begin{figure*}
\centering     %%% not \center
\subfigure[]{\label{fig:neuron_transform_1FI}\includegraphics[width=0.91\linewidth]{images/curated_plots_layer_wise/neurons_1FI_transformer.png}}
\vspace{-0.25cm} 
\subfigure[]{\label{fig:neuron_CNN_1FI}\includegraphics[width=0.91\linewidth]{images/curated_plots_layer_wise/neurons_1FI_cnns.png}}
\vspace{-0.25cm} 
\subfigure[]{\label{fig:weight_transform_1FI}\includegraphics[width=0.91\linewidth]{images/curated_plots_layer_wise/weights_1FI_transformer.png}}
\vspace{-0.25cm} 
\subfigure[]{\label{fig:weight_CNN_1FI}\includegraphics[width=0.91\linewidth]{images/curated_plots_layer_wise/weights_1FI_cnns.png}}
\vspace{-0.25cm} 
% \vspace{-0.25cm} 
\caption{Single bit flip error transformers and CNN-based object detection models.}
\label{fig:single_bit_flip}
\end{figure*}



\begin{figure*}
\centering     %%% not \center
\subfigure[]{\label{fig:neuron_transform_10FI}\includegraphics[width=0.91\linewidth]{images/curated_plots_layer_wise/neurons_10FI_transformer.png}}
\vspace{-0.25cm} 
\subfigure[]{\label{fig:neuron_CNN_10FI}\includegraphics[width=0.91\linewidth]{images/curated_plots_layer_wise/neurons_10FI_cnns.png}}
\vspace{-0.25cm} 
\subfigure[]{\label{fig:weight_transform_10FI}\includegraphics[width=0.91\linewidth]{images/curated_plots_layer_wise/weights_10FI_transformer.png}}
\vspace{-0.25cm} 
\subfigure[]{\label{fig:weight_CNN_10FI}\includegraphics[width=0.91\linewidth]{images/curated_plots_layer_wise/weights_10FI_cnns.png}}
\vspace{-0.25cm} 
\caption{10-bit flip error transformers and CNN-based object detection models.}
\label{fig:10_bit_flips}
\end{figure*}

% \begin{figure*}
% \centering     %%% not \center
% \subfigure[]{\label{fig:dino_detr_ap50}\includegraphics[width=0.91\linewidth]{images/curated_plots_layer_wise/neurons_1FI_transformer.png}}
% \vspace{-0.25cm} 
% \subfigure[Layer monitoring after fault injection]{\label{fig:dino_detr_sdc}\includegraphics[width=0.91\linewidth]{images/curated_plots_layer_wise/weights_1FI_transformer.png}}
% % \vspace{-0.25cm} 
% \caption{Single bit flip error transformers.}
% \label{fig:dino_detr_sdc_ap50}
% \end{figure*}


% \begin{figure*}
% \centering     %%% not \center
% \subfigure[]{\label{fig:dino_detr_ap50}\includegraphics[width=0.91\linewidth]{images/curated_plots_layer_wise/neurons_10FI_transformer.png}}
% \vspace{-0.5cm}
% \subfigure[Layer monitoring after fault injection]{\label{fig:dino_detr_sdc}\includegraphics[width=0.91\linewidth]{images/curated_plots_layer_wise/weights_10FI_transformer.png}}
% \caption{10-bit flip error transformers.}
% \label{fig:dino_detr_sdc_ap50}
% \end{figure*}

% \begin{figure*}
% \centering     %%% not \center
% \subfigure[]{\label{fig:dino_detr_ap50}\includegraphics[width=0.91\linewidth]{images/curated_plots_layer_wise/neurons_1FI_cnns.png}}
% \vspace{-0.5cm}
% \subfigure[Layer monitoring after fault injection]{\label{fig:dino_detr_sdc}\includegraphics[width=0.91\linewidth]{images/curated_plots_layer_wise/weights_1FI_cnns.png}}
% \caption{Single bit flip error CNNs.}
% \label{fig:dino_detr_sdc_ap50}
% \end{figure*}

==> sec_new/abstract.tex <==
\begin{abstract}

As transformer-based object detection models advance, their influence within the computer vision field is anticipated to expand, particularly in safety-critical domains like autonomous vehicles and aviation. Soft errors, leading to bit flips in the weights or neurons of the model during inference, have notably affected DNN performance by changing predictions. The existing range restriction solutions, initially designed for CNN-based models, are not directly applicable to transformer-based models. This study introduces Global Clipper and Global Hybrid Clipper, offering a straightforward yet effective mitigation approach tailored for transformer-based object detection models. These solutions enhance the overall resilience of these models against soft errors, reducing faulty inferences to ~ 0\%. Additionally, we conduct a comprehensive set of experiments involving over 64 scenarios on two transformer-based (DINO-DETR and Lite-DETR) and two CNN-based object detection models (YOLOv3 and SSD) using three datasets, amounting to $~$3.3 million inferences, to provide a detailed understanding of the robustness of these models. Furthermore, the paper highlights the fundamental characteristics of different attention blocks in transformers and discusses behavioural differences compared to CNNs.
\end{abstract}



% As transformer-based object detection models continue to evolve and mature, their impact on the computer vision field is expected to grow even further, especially in safety-critical domains. Soft errors induce bit flips which have been proved to impact the DNN performance by altering the predictions significantly. The existing range restriction solutions originally proposed for CNN-based models do not work off the shelf for the transformer-based models. In this work, we propose Global Clipper and Global Hybrid Clipper  - a simple and effective mitigation solution for transformer-based object detection built on top of existing range restriction algorithms. It enhances the overall resiliency of these models against soft errors by reducing the faulty inferences from 3\% to 0\%. Furthermore, we conduct more than 64 sets of a large set of experiments on two transformer-based and CNN-based object detection models totalling $~$ 3.3 million inferences to understand the robustness of these models in detail.
